p-multigrid method for the discontinuous Galerkin discretization of elliptic problems

In this paper, we propose a $W$-cycle $p$-multigrid method for solving the $p$-version symmetric interior penalty discontinuous Galerkin (SIPDG) discretization of elliptic problems. This SIPDG discretization employs hierarchical Legendre polynomial basis functions. Inspired by the uniform convergence theory of the $W$-cycle $hp$-multigrid method in [P. F. Antonietti, et al., SIAM J. Numer. Anal., 53 (2015)], we provide a rigorous convergence analysis for the proposed $p$-multigrid method, considering both inherited and non-inherited bilinear forms of SIPDG discretization. Our theoretical results show significant improvement over [P. F. Antonietti, et al., SIAM J. Numer. Anal., 53 (2015)], reducing the required number of smoothing steps from $O(p^2)$ to $O(p)$, where $p$ is the polynomial degree of the discrete broken polynomial space. Moreover, the convergence rate remains independent of the mesh size. Several numerical experiments are presented to verify our theoretical findings. Finally, we numerically verify the effectiveness of the $p$-multigrid method for unfitted finite element discretization in solving elliptic interface problems on general $C^{2} $-smooth interfaces.

==> error.tex <==

\subsection{Stability analysis and error estimates}
Before describing our $p$-multigrid method,
we will show some basic numerical analysis for the IPDG discretizations
without proof.

Based on these assumptions, we define the DG energy norm as
\begin{equation}\label{DG_norm}
||v||_{DG}^2 := \sum\limits_{K\in \mathcal{T}_h} ||a^{\frac{1}{2}}\nabla v||^2_{L^2(K)}
+ \sum\limits_{e\in \mathcal{E}_h}||\alpha^{\frac{1}{2}} \llbracket v \rrbracket||_{L^2(e)}^2,
\quad \forall v\in U_p(\Ct_h). \\
\end{equation}



We proceed to demonstrate that the bilinear form $a_{DG}(\cdot, \cdot)$
as defined in \eqref{IPDG_a}, exhibits continuity and coerciveness
in the context of the DG energy norm \eqref{DG_norm}
within the discrete piecewise polynomial space $U_p(\Ct_h)$.

\begin{lemma}\label{lemma1}
	There exists constants $C_{stab}, C_{cont} > 0$ independent on
	the degree of the discrete polynomial space $U_p(\Ct_h)$, the penalty parameters $\alpha$,
	and the mesh size $h$ such that,
	\begin{eqnarray}
		&|a_{DG}(u,v)| \leq C_{cont} ||u||_{DG}||v||_{DG}, \quad &\forall u,v\in U_p(\Ct_h), \label{lemma_cont}\\
		&a_{DG}(v,v) \geq C_{stab} ||v||^2_{DG}, \quad &\forall v\in U_p(\Ct_h). \label{lemma_stab}
	\end{eqnarray}
\end{lemma}

\begin{proof}
For any $v\in U_p(\Ct_h)$, we have
$$a_{DG}(v,v) = ||v||^2_{DG}
- 2 \sum\limits_{e\in \mathcal{E}_h} \int_e  \left\{\!\left\{a \frac{\partial v}{\partial \boldsymbol{n}_e} \right\}\!\right\} \llbracket v\rrbracket d s.$$
Apply the Young's inequality, we have
\begin{equation*}
\begin{aligned}
\sum\limits_{e\in \mathcal{E}_h} \int_e  \left\{\!\left\{a \frac{\partial v}{\partial \boldsymbol{n}_e} \right\}\!\right\} \llbracket v\rrbracket d s
&\leq& &\frac{1}{2\varepsilon}\sum\limits_{e\in \mathcal{E}_h} \int_e  \left\{\!\left\{a \frac{\partial v}{\partial \boldsymbol{n}_e} \right\}\!\right\}^2 d s
+ \frac{\varepsilon a_M}{2}\sum\limits_{e\in \mathcal{E}_h} \int_e \llbracket v\rrbracket^2 d s \\
\end{aligned}
\end{equation*}
and with local trace inequality we have
$$\sum\limits_{e\in \mathcal{E}_h} \int_e \left\{\!\left\{a \frac{\partial v}{\partial \boldsymbol{n}_e} \right\}\!\right\}^2 d s
\leq \frac{Cp^2}{h}\sum\limits_{K\in \mathcal{T}_h}\int_K a\nabla v\cdot \nabla v d\Omega
= \frac{Cp^2}{h}\sum\limits_{K\in \mathcal{T}_h}\|a^{\frac{1}{2}}\nabla v \|^2_{L^2(K)}.$$

Take $\varepsilon = \frac{Cp^2}{h}$,
\begin{equation}
\begin{aligned}
a_{DG}(v,v)
&\geq& &||v||_{DG}^2 - \frac{1}{2\varepsilon}\sum\limits_{e\in \mathcal{E}_h} \int_e  \left\{\!\left\{a \frac{\partial v}{\partial \boldsymbol{n}_e} \right\}\!\right\}^2 d s
- \frac{\varepsilon a_M}{2}\sum\limits_{e\in \mathcal{E}_h} \int_e \llbracket v\rrbracket^2 d s \\
&\geq& &||v||_{DG}^2 - \frac{Cp^2 }{2\varepsilon h}\sum\limits_{K\in \mathcal{T}_h} ||a\nabla v ||^2_{L^2(K)}
- \frac{\varepsilon a_M}{2}\sum\limits_{e\in \mathcal{E}_h} \int_e \llbracket v\rrbracket^2 d s \\
&=& &||v||_{DG}^2 - \frac{1}{2}\sum\limits_{K\in \mathcal{T}_h} ||a\nabla v ||^2_{L^2(K)}
- \frac{Cp^2 a_M}{2h}\sum\limits_{e\in \mathcal{E}_h} \int_e \llbracket v\rrbracket^2 d s \\
&\geq& &||v||_{DG}^2 - \max \left\{\frac{1}{2}, \frac{C}{2\alpha_0} \right\} ||v||^2_{DG}
\end{aligned}
\end{equation}
then we have $a_{DG}(v,v)\geq C_{stab}||v||^2_{DG}$ when $\alpha_0$ is big enough.


For \eqref{lemma_cont}, we have
\begin{equation*}
\begin{aligned}
a_{DG}(u, v) &\leq& &\left| \sum\limits_{K\in \mathcal{T}_h}\int_{K}a \nabla u\cdot \nabla v d\Omega \right| \\
&& + & \left| \sum\limits_{e\in \mathcal{E}_h} \int_e \left( \left\{\!\left\{a \frac{\partial u}{\partial \boldsymbol{n}_e} \right\}\!\right\} \llbracket v\rrbracket
+ \left\{\!\left\{a \frac{\partial v}{\partial \boldsymbol{n}_e}\right\}\!\right\}\llbracket u\rrbracket  \right) d s \right|\\
&& + &\left| \sum\limits_{e\in \mathcal{E}_h} \int_e \alpha \llbracket u\rrbracket \llbracket v\rrbracket d s \right|  \\
&\leq & &C_{cont} ||u||_{DG}||v||_{DG},
\end{aligned}
\end{equation*}
and one can also refer to \cite{Prudhome2000, Hartmann2009} for details.

\end{proof}

Importantly, these constants $C_{stab}, C_{cont}$ holds
regardless of the mesh size $h$ and the diffusion coefficients $a(\boldsymbol{x})$.
It should be highlighted that the stability property
is also dependent on the penalty parameter $\alpha$ in \eqref{IPDG_a}.
which must be selected in a manner that is sufficiently large
to guarantee the stability of the bilinear form $a_{DG}(\cdot, \cdot)$.




Moreover, without the proof,
we have the following error estimates \cite{Antonietti2015},
$hp$ inverse estimates \cite{Schwab1998}
and condition number estimates \cite{Hu1998,Olsen1995}.

\begin{lemma}
Assume the exact solution $u$ satisfies $u\in H^{s+1}(\Omega)$ with $s\geq 1$,
we have the following error estimates
\begin{eqnarray}
||u-u_h||_{DG} &\leq& C\frac{h^{\min(p,s)}}{p^{s-1/2}}||u||_{H^{s+1}} \\
||u-u_h||_{L^2(\Omega)} &\leq& C\frac{h^{\min(p,s)+1}}{k^{s}}||u||_{H^{s+1}}
\end{eqnarray}
where $C$ is constant independent of $p, h, a(\boldsymbol{x})$.
\end{lemma}

\begin{lemma}
Let $K\in \mathcal{T}$, then we have
\begin{eqnarray*}
||\nabla v||_{L^2(K)} \leq Cp^2h^{-1}||v||_{L^2(K)}, \quad \forall v\in U_p(\Ct_h) \\
||v||_{L^2(\partial K)} \leq C p h^{-1/2}||v||_{L^2(K)}, \quad \forall v\in U_p(\Ct_h)
\end{eqnarray*}
where $C$ is independent of $h$ and $p$.
\end{lemma}








%%%
